Anisotropy of the proton kinetic energy as a tool for capturing structural transition in nanoconfined H$_2$O

The proton dynamics of a 2D water monolayer confined inside a graphene slit pore is studied in Cartesian and molecular frames of reference using molecular dynamics simulations. The vibrational density of states of the proton was calculated versus temperature and was further used to deduce the mean kinetic energy of the hydrogen atoms, Ke(H), in both frames of reference. The directional components of Ke(H) are in good agreement with experimental observations for bulk as well as nanoconfined water. Nonetheless, while in the molecular frame of reference the effect of temperature on the anisotropy ratios of Ke(H) (the ratio between its directional components) are practically invariant between the 2D and 3D cases, those in the Cartesian frame of reference reveal a rather notable reduction across 200K, indicating the occurrence of an order-disorder transition. This result is further supported by the calculated entropy and enthalpy of the confined water molecules. Overall it is shown that Ke(H) anisotropy ratios may serve as a valuable order parameter for detecting structural transformations in hydrogen bonds containing molecular systems.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
